Hyperbolic Geometric Latent Diffusion Model for Graph Generation

Diffusion models have made significant contributions to computer vision, sparking a growing interest in the community recently regarding the application of them to graph generation. Existing discrete graph diffusion models exhibit heightened computational complexity and diminished training efficiency. A preferable and natural way is to directly diffuse the graph within the latent space. However, due to the non-Euclidean structure of graphs is not isotropic in the latent space, the existing latent diffusion models effectively make it difficult to capture and preserve the topological information of graphs. To address the above challenges, we propose a novel geometrically latent diffusion framework HypDiff. Specifically, we first establish a geometrically latent space with interpretability measures based on hyperbolic geometry, to define anisotropic latent diffusion processes for graphs. Then, we propose a geometrically latent diffusion process that is constrained by both radial and angular geometric properties, thereby ensuring the preservation of the original topological properties in the generative graphs. Extensive experimental results demonstrate the superior effectiveness of HypDiff for graph generation with various topologies.

==> 3_preliminary.tex <==

\section{Preliminary}
In this section, we briefly introduce some notations and key definitions. 
Our work focuses on the relationship between labeled node imbalance and hierarchical geometric properties of graphs in the semi-supervised node classification task on graphs. 
Therefore, let us revisit the unbalanced semi-supervised node classification and the hyperbolic geometric model. 

\subsection{Discrete Graph Denoising Diffusion model}
Given a graph $\mathcal{G}=\{\mathcal{V},\mathcal{E}\}$ with the node set  $\mathcal{V}$ of $N$ nodes and the edge set $\mathcal{E}$.  
Let $\mathbf{A}\in \mathbb{R}^{N\times N}$ be the adjacency matrix and $\mathbf{X}\in \mathbb{R}^{N\times d}$ be the node feature matrix, where $d$ denotes the dimension of node features. 
For node $v$, its neighbors set is $N (v): \{u \in \mathcal{V} |u, v \in \mathcal{E}\}. 
$ $d_v : |\mathcal{N} (v)|$ is the degree of node $v$.
Given the labeled node set $\mathcal{V}_L$ and their labels $\mathcal{Y}_L$ where each node $v_i$ is associated with a label $y_i$, \textit{semi-supervised node classification} aims to train a node classifier $f_{\theta}:v\rightarrow\mathbb{R}^{C}$ to predict the labels $\mathcal{Y}_U$ of remaining unlabeled nodes $\mathcal{V}_U=\mathcal{V} \setminus \mathcal{V}_L$, where $C$ denotes the number of classes. 
We separate the labeled node set $\mathcal{V}_L$ into $\{\mathcal{V}^{1}_L, \mathcal{V}^2_L, \cdots, \mathcal{V}^{C}_L\}$, where $\mathcal{V}^i_L$ denotes the nodes of class $i$ in $\mathcal{V}_L$. 

We focus on the semi-supervised node classification based on GNNs, which is a powerful and widely used graph representation learning model.
GNNs are composed of message $\operatorname{M}$ and update function $\operatorname{U}$ in the message-passing paradigm, and the $l$th-GNNs layer is defined as: 
\begin{equation}\label{equ:GNN_layer}
   \begin{aligned}
    \boldsymbol{h}_{i}^{l+1} &=\operatorname{U}^{l}\left(\boldsymbol{h}_{i}^{l}, \sum_{j \in \mathcal{N}(i)} \operatorname{M}^{l}\left(\boldsymbol{h}_{i}^{l}, \boldsymbol{h}_{j}^{l}, e_{i j}\right)\right),
    \end{aligned}
\end{equation}
where $e_{i j}$ is the edge of nodes $\{v, u\} \in \mathcal{E}$.


\subsection{Hyperbolic Geometric Model}
Hyperbolic space commonly refers to a manifold with constant negative curvature and is used for modeling complex networks. 
In hyperbolic geometry, five common isometric models are used to describe hyperbolic spaces~\cite{cannon1997hyperbolic}. 
Among them, the Poincaré model has recently been introduced into machine learning for preserving the hierarchy of graphs. 
In this work, we use the Poincar{\'{e}} disk model to reveal the underlying hierarchy of the graph. 

\begin{myDef}[Poincar{\'{e}} disk Model]
	\label{def:poincare}
    The Poincar\'e Disk Model is a two-dimensional model of hyperbolic geometry with nodes located in the unit disk interior, and the generalization of n-dimensional with standard negative curvature $c$ is the Poincar\'e ball $\mathcal{B}^{n}_{c} = \{\boldsymbol{x} \in \mathbb{R}^n: \left\| \boldsymbol{x} \right\|^2 < 1/c \}$. For any point pair $(\boldsymbol{x}, \boldsymbol{y}) \in \mathcal{B}^{n}_c$, $\boldsymbol{x} \ne \boldsymbol{y}$, the distance on this manifold is defined as:
    \begin{equation}\label{Eq:hyperbolic_distance}
        d_{\mathcal{B}^{n}_{c}}(\boldsymbol{x}, \boldsymbol{y}) = \frac{2}{\sqrt{c}} \tanh^{-1} (\sqrt{c} \left\| -\boldsymbol{x} \oplus_c \boldsymbol{y} \right\|),
    \end{equation}
    where $\oplus_c$ is M\"{o}bius addition and $\left\| \cdot \right\|$ is $L_2$ norm.
\end{myDef}

\begin{myDef}[Poincar\'e norm]\label{def:Poincare_norm}
The Poincar{\'{e}} Norm is defined as the distance of any point $\boldsymbol{x} \in \mathcal{B}^{n}_{c}$ from the origin of Poincar{\'{e}} ball:
\begin{equation}
\label{Eq:distortion}
\left\| \boldsymbol{x} \right\|_{\mathcal{B}^{n}_{c}} = \frac{2}{\sqrt{c}} \tanh^{-1} (\sqrt{c} \left\| \boldsymbol{x} \right\|).
\end{equation}
\end{myDef}
% \begin{myDef}[Exponential and Logarithmic Maps]
%     The manifold $\mathcal{M}^d$ and the tangent space $\mathcal{T}_{\mathrm{x}}$ can be mapped to each other via \textit{exponential map} and \textit{logarithmic map}. 
%     The \textit{exponential map} $\mathrm{exp}_{\mathbf{x}}^{c}(\cdot)$ and \textit{logarithmic map} $\log _{\mathbf{x}}^{c}(\cdot)$ are defined as: 
%     \begin{equation}\label{log_exp_mapping}
%     \begin{aligned}
%         & \exp_{\boldsymbol{x}}^c(\boldsymbol{v}) = \boldsymbol{x} \oplus_c \frac{1}{\sqrt{c}} \tanh \left( \frac{\sqrt{c}\lambda_{\boldsymbol{x}}^c \left\| \boldsymbol{v} \right\|}{2} \right) \frac{\boldsymbol{v}}{\left\| \boldsymbol{v} \right\|}, \\
%         &\log_{\boldsymbol{x}}^c(\boldsymbol{u}) = \frac{2}{\sqrt{c}\lambda_{\boldsymbol{x}}^c} \tanh^{-1} \left( \sqrt{c} \left\| - \boldsymbol{x} \oplus_c \boldsymbol{u} \right\| \right) \frac{- \boldsymbol{x} \oplus_c \boldsymbol{u}}{\left\| - \boldsymbol{x} \oplus_c \boldsymbol{u} \right\|},
%     \end{aligned}
%     \end{equation}
%     where $\oplus_c$ is M\"{o}bius addition.
% \end{myDef}
 


